Matching for causal effects via multimarginal unbalanced optimal transport

Matching on covariates is a well-established framework for estimating causal effects in observational studies. The principal challenge stems from the often high-dimensional structure of the problem. Many methods have been introduced to address this, with different advantages and drawbacks in computational and statistical performance as well as interpretability. This article introduces a natural optimal matching method based on multimarginal unbalanced optimal transport that possesses many useful properties in this regard. It provides interpretable weights based on the distance of matched individuals, can be efficiently implemented via the iterative proportional fitting procedure, and can match several treatment arms simultaneously. Importantly, the proposed method only selects good matches from either group, hence is competitive with the classical k-nearest neighbors approach in terms of bias and variance in finite samples. Moreover, we prove a central limit theorem for the empirical process of the potential functions of the optimal coupling in the unbalanced optimal transport problem with a fixed penalty term. This implies a parametric rate of convergence of the empirically obtained weights to the optimal weights in the population for a fixed penalty term.

==> Florian/Thm1_alternative.tex <==
\begin{proof}
We want to derive the asymptotic probability measure of the empirical process
\begin{align*}
    &\sqrt{N}\left( \int f(x) \dd\hat\gamma_N(x) - \int f(x) \dd\gamma(x)  \right)\\
    =&\sqrt{N}\left(\int f(x) \exp\left(\frac{\sum_{j=1}^J\hat\varphi_{N_j}-c}{\varepsilon}\right)\dd\bigotimes_j\hat\mu_{N_j} - \int f(x) \exp\left(\frac{\sum_{j=1}^J\varphi_j^*-c}{\varepsilon}\right)\dd\bigotimes_j\mu_j  \right),
\end{align*}
which is an empirical process indexed by estimated functions \citep{wellner2007empirical}.
For notational convenience we use the empirical process notation 
\[\mathbb{P}_N f=\int f(x) \dd\bigotimes_{j=1}^J\hat\mu_{N_j}(x),\qquad\mathbb{P} f=\int f(x) \dd\bigotimes_{j=1}^J\mu_{_j}(x),\qquad\mathbb{G}_Nf = \sqrt{N}(\mathbb{P}_Nf-\mathbb{P}f)\] and write
\[\sqrt{N}\left(\mathbb{P}_N f \hat{K}_N - PfK\right) 
= \mathbb{G}_N\left(f \hat{K}_N - fK\right) + \mathbb{G}_NfK + \sqrt{N}P\left(f \hat{K}_N - fK\right).\]

We proceed term by term. We first show that the first term is asymptotically negligible, i.e.~$\mathbb{G}_N \left(\hat K_Nf -Kf\right) = o_P(1)$. For this we have to verify the conditions in Lemma 19.24 in \cite{van2000asymptotic}.
Similar to the proof of Lemma \ref{lem:potential}, we define the following class of functions
\begin{align*}
    \tilde{\mathcal{F}}_{Kf}\coloneqq\left\{\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right) f \right]: \thickspace \right. \left.\thickspace \varphi\in \prod_jC^\infty(\mathcal{X}_j), f\in \mathcal{F}\right\},
\end{align*}
where $\mathcal{F}$ is some uniformly bounded Donsker class on $\prod_j\mathcal{X}_j$ by assumption. Using the same argument as in Lemma \ref{lem:potential}, we split this class into 
\[\tilde{\mathcal{K}}_{K}\coloneqq\left\{\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right) \right]:\thickspace \right. \left.\thickspace \varphi\in \prod_jC^\infty(\mathcal{X}_j)\right\}\qquad\text{and}\qquad \mathcal{F}.\] The first term has a bounded bracketing entropy integral since the exponential function is smooth. Moreover, due to the compactness of $\mathcal{X}_j$ and smoothness of functions in $\tilde{\mathcal{K}}_{\delta,K}$ it is also uniformly bounded and hence a uniformly bounded $\mathbb{P}$-Donsker class. Since the product of two uniformly bounded Donsker classes is a Donsker class by Example 2.10.8 in \cite{wellner2013weak}, this implies that $\tilde{\mathcal{F}}_{\delta,Kf}$ is also $\mathbb{P}$-Donsker. We also need to show that 
\begin{equation}\label{eq:quadconv}P\left(\hat{K}_Nf - Kf\right)^2 = o_P(1).\end{equation}
This follows from the following bound.
\begin{align*}
&\left\lvert \exp\left(\frac{\sum_j\varphi_j-c}{\varepsilon}\right) -\exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon} \right)\right\rvert\\
=& \left\lvert \exp\left(\frac{\sum_j\varphi_j^*-c}{\varepsilon}\right)\left[ \exp\left(\frac{\sum_j\varphi_j-\varphi^*_j}{\varepsilon}\right) -1\right]\right\rvert\\
\leq& \exp\left(\frac{\sum_j\left\|\varphi_j^*\right\|_\infty-c}{\varepsilon}\right)\left\lvert \exp\left(\frac{\sum_j\left\|\varphi_j-\varphi^*_j\right\|_\infty}{\varepsilon}\right) -1\right\rvert.
\end{align*}
Taking the supremum over $\prod_j\mathcal{X}_j$ on both sides gives
\begin{align*}
    &\left\| \exp\left(\frac{\sum_j\varphi_j-c}{\varepsilon}\right) -\exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon} \right)\right\|_\infty\\\leq& \exp\left(\frac{\sum_j\left\|\varphi_j^*\right\|_\infty-c}{\varepsilon}\right)\left\lvert \exp\left(\frac{\sum_j\left\|\varphi_j-\varphi^*_j\right\|_\infty}{\varepsilon}\right) -1\right\rvert.
    \end{align*}
This implies that the LHS is bounded, because the RHS is by assumption bounded. Therefore, by the boundedness of $f$, H\"older's inequality in conjunction with the consistency of the potentials from Lemma \ref{lem:consistency} implies \eqref{eq:quadconv}. 

Therefore, by Lemma 19.24 in \citet{van2000asymptotic} or Lemma 3.3.5 in \citet{wellner2013weak} the first term is uniformly asymptotically negligible, i.e.
\begin{equation}\label{eq:asyneg}
\sup_{f\in\mathcal{F}}\left\lvert\mathbb{G}_N\left(\hat{K}_Nf-Kf\right)\right\rvert = o_{P^*}\left(1+\sqrt{N}\|\hat{\varphi}^m_N-\varphi^*\|_{C^\infty}\right).
\end{equation}

Now focus on the second and third term jointly. The second term is a standard empirical process over a Donsker class which converges to a tight mean-zero Gaussian process. The third term also converges to a tight Gaussian process by the Continuous Mapping Theorem \citep[Theorem 1.11.1]{wellner2013weak} and Proposition \ref{prop:density}, where we showed weak convergence to a tight mean-zero Gaussian process.

Both weak convergence results are for the marginal distributions, not the joint distribution, however. So in order to conclude that the sum of the last two terms converges to a tight Gaussian process, we need show that their joint distribution converges to a joint tight Gaussian process. 

Let us write out both terms explicitly. 
\begin{align*}
    &\mathbb{G}_NfK = \sqrt{N}\int f\exp\left(\frac{\sum_{j=1}^J \varphi_j^*-c}{\varepsilon}\right)\dd\left[\bigotimes_j\hat{\mu}_{N_j} -\bigotimes_j\mu_j\right]\qquad\text{and} \\
    &\sqrt{N}P\left(f \hat{K}_N - fK\right) = \sqrt{N}\int f\left[\exp\left(\frac{\sum_{j=1}^J \hat\varphi^m_{N_j}-c}{\varepsilon}\right) - \exp\left(\frac{\sum_{j=1}^J \varphi_j^*-c}{\varepsilon}\right)\right]\dd\bigotimes_j\mu_j
\end{align*}

\ndfg{Finish this.}
We now show that the sum of these terms is asymptotically equal to a Gaussian process. Since $\varphi^*$ is a $Z$-estimator, it holds
\[\delta F(\varphi^*,v) = 0\qquad\text{and}\qquad \delta\hat{F}_N(\hat{\varphi}^m_N,v) = o_P(N^{-\frac{1}{2}})\] for all $v\in \prod_j B_1\left(C^\infty_c(\mathcal{X}_j)\right)$, where the latter follows by choosing a large enough $m$ in generalized Sinkhorn algorithm, which is always possible by Lemma \ref{lem:consistency}. Since smooth functions are dense in the space of integrable functions, it also holds that
\[\delta F(\varphi^*,f)=0\qquad\text{and}\qquad \delta\hat{F}_N(\hat{\varphi}_N^m,f) = o_P(N^{-\frac{1}{2}})\] uniformly over $f\in\mathcal{F}$. Then 
\[\sqrt{N}\left(\delta F(\hat{\varphi}_N^m,f) - \delta F(\varphi^*,f)\right) = \sqrt{N}\left(\delta F(\hat{\varphi}_N^m,f) - \delta \hat{F}_N(\hat{\varphi}^m_N,f)\right)+o_P(1).\] 


Moreover, by Lemma 3.3.5 in \citet{wellner2013weak} and the above argument, the second term satisfies
\[\sqrt{N}\left(\delta F(\hat{\varphi}^m_N,f) - \delta\hat{F}_N(\hat{\varphi}_N^m,f)\right) = -\sqrt{N}\left(\delta\hat{F}_N(\varphi^*,f) - \delta F(\varphi^*,f)\right) +o_P(1+\sqrt{N}\|\hat{\varphi}_N^m - \varphi^*\|_{C^\infty}).\]
Putting both together gives
\begin{multline*}
    \sqrt{N}\left(\delta F(\hat{\varphi}_N^m,f) - \delta F(\varphi^*,f)\right) \\= -\sqrt{N}\left(\delta\hat{F}_N(\varphi^*,f) - \delta F(\varphi^*,f)\right) +o_P(1+\sqrt{N}\|\hat{\varphi}_N^m - \varphi^*\|_{C^\infty}) + o_P(1).
\end{multline*}

But recall that
\[\delta\hat{F}_N(\varphi^*,f) = \int f\left[\exp\left(\frac{\sum_j\varphi_j -c}{\varepsilon}\right)-1\right]\dd\bigotimes_j\hat{\mu}_{N_j}\] and similar for all other terms. 
Therefore,
\begin{align*}
    &\sqrt{N}\left(\delta F(\hat{\varphi}_N^m,f) - \delta F(\varphi^*,f)\right) \\=& \int f\left[\exp\left(\frac{\sum_j\hat{\varphi}_{N_j}^m - c}{\varepsilon}\right) - \exp\left(\frac{\sum_j\varphi^* - c}{\varepsilon}\right)\right]\dd\bigotimes_j\mu_j \\=& \sqrt{N}P\left(f \hat{K}_N - fK\right)
\end{align*}
Similarly, 
\begin{align*}
    &\sqrt{N}\left(\delta \hat{F}_N(\varphi^*,f) - \delta F(\varphi^*,f)\right) \\=& \int f\left[\exp\left(\frac{\sum_j\varphi^* - c}{\varepsilon}\right)-1\right]\dd\left[\bigotimes_j\hat\mu_{N_j} - \bigotimes_j\mu_j\right] \\=& \mathbb{G}_NfK - \mathbb{G}_Nf.
\end{align*}
Therefore,
\[\mathbb{G}_NfK + \sqrt{N}P\left(f \hat{K}_N - fK\right)= \mathbb{G}_Nf +o_P(1+\sqrt{N}\|\hat{\varphi}_N^m - \varphi^*\|_{C^\infty}) + o_P(1).\]

Putting everything together we have
\begin{align*}
&\sqrt{N}\left(\mathbb{P}_N f \hat{K}_N - PfK\right) \\
=& \mathbb{G}_N\left(f \hat{K}_N - fK\right) + \mathbb{G}_NfK + \sqrt{N}P\left(f \hat{K}_N - fK\right)\\
=& o_P(1) +\mathbb{G}_Nf + o_P(1+\sqrt{N}\|\hat{\varphi}_N^m - \varphi^*\|_{C^\infty}) + o_P(1).
\end{align*}
Since $f$ lies in a bounded Donsker class by our assumption, it follows that the corresponding limit process of $\sqrt{N}\left(\mathbb{P}_N f \hat{K}_N - PfK\right) $ is a mean zero tight Gaussian process with covariance $P(f_1f_2) - Pf_1Pf_2$. The conclusion of Theorem 3.6.1 in \citet{wellner2013weak} also implies that the standard bootstrap works.
\end{proof}

==> Old versions/old_simulation.tex <==
\section{Illustration}\label{sec:illu}
The excellent statistical finite-sample properties of the proposed method, especially compared to the standard $k$-nearest neighbor approach \citep{abadie2004implementing}, can already be appreciated in simple two-dimensional simulation studies. We propose two simulations, one with Gaussian distributions and one with a simple mixture of two Gaussians. To compare the method to the existing nearest neighbor approach, we focus on pairwise matchings. 
\begin{figure}
\centering
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plot/before_mapping_ellipse.pdf}
  \caption{Covariates 95\% quantile before mapping. }
  \label{fig:ellipse_before}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plot/after_mapping_ellipse.pdf}
  \caption{Covariates 95\% quantile after mapping.}
  \label{fig:ellipse_after}
\end{subfigure}
\vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/before_mapping_scatter.pdf}
            \caption[]%
            {{\small Scatter plot before mapping}}    
            \label{fig:scatter_before_mapping}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/after_mapping_scatter.pdf}
            \caption[]%
            {{\small Scatter plot after mapping}}    
            \label{fig:scatter_after_mapping}
        \end{subfigure}
        \vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/mixture_before.pdf}
            \caption[]%
            {{\small Mixtures of 2 Gaussians before mapping}}    
            \label{fig:mixture_before_mapping}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/mixture_after.pdf}
            \caption[]%
            {{\small Mixtures of 2 Gaussians after mapping}}    
            \label{fig:mixture_after_mapping}
        \end{subfigure}
\caption{Covariates plot before and after matching. 95\% quantile ellipses are computed based on estimated mean vector and covariance matrix on each sample.}
\label{fig:matching_scatter}
\end{figure}

For the first simulation, we sample 3 groups of covariates, denoted as $X_0,X_1,X_2$, and match both $X_1$ and $X_2$ to $X_0$. The 3 groups of covariates are sampled from bivariate normal distributions as follows.

\begin{align*}
    &\mathbf{X}_0\sim N\left\{ \left(\begin{array}{c}
         1\\0
    \end{array}\right),\left(\begin{array}{cc}
        1 & 0 \\
        0 & 1
    \end{array}\right)\right\},~
    \mathbf{X}_1\sim N\left\{ \left(\begin{array}{c}
         0.5\\-0.2
    \end{array}\right),\left(\begin{array}{cc}
        1 & 0.1 \\
        0.1 & 1
    \end{array}\right)\right\},\\
    &\mathbf{X}_2\sim N\left\{ \left(\begin{array}{c}
         0.7\\-0.2
    \end{array}\right),\left(\begin{array}{cc}
        0.5 & 0.1 \\
        0.1 & 0.5
    \end{array}\right)\right\}
\end{align*}

For the second simulation, the 3 groups of covariates are denoted by $Z_0,Z_1$ and $Z_2$ respectively. Each of them follows a mixture distribution of 2 Gaussians, where $Z_0\sim 0.7X_0+0.3X_1$, $Z_1\sim 0.5X_1+0.5X_3$, and $Z_2\sim 0.6X_2+0.4X_3$. In Figures \ref{fig:matching_scatter}, \ref{fig:ellipse_before} and \ref{fig:ellipse_after} we plot the 95\% elliptic contour of the bivariate normal distributions for each group before and after matching, based on the mean and covariate matrix estimated from each sample, whereas \ref{fig:scatter_before_mapping} and \ref{fig:scatter_after_mapping} give the scatter plots.
\begin{figure}
\centering
\begin{subfigure}{0.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plot/kmeans_ellipse_before.pdf}
  \caption{Covariates 95\% quantile before mapping. }
  \label{fig:kmeans_ellipse_before}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=\textwidth]{plot/kmeans_ellipse_after.pdf}
  \caption{Covariates 95\% quantile after mapping.}
  \label{fig:kmeans_ellipse_after}
\end{subfigure}
\vskip\baselineskip
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/kmeans_scatter_before.pdf}
            \caption[]%
            {{\small Scatter plot before mapping}}    
            \label{fig:kmeans_scatter_before}
        \end{subfigure}
        \hfill
        \begin{subfigure}[b]{0.475\textwidth}   
            \centering 
            \includegraphics[width=\textwidth]{plot/kmeans_scatter_after.pdf}
            \caption[]%
            {{\small Scatter plot after mapping}}    
            \label{fig:kmeans_scatter_after}
        \end{subfigure}
\caption{Covariates plot before and after $k$-nearest neighbors matching, $k=3$. 95\% quantile ellipses are computed based on estimated mean vector and covariance matrix on each sample.}
\label{fig:kmeans_plot}
\end{figure}

In both simulations, we sample $N_0=70, N_1=60, N_2 = 80$ points from each group respectively. The simulation is performed using the \texttt{POT} python package \citep{flamary2021pot}. Figure \ref{fig:mixture_before_mapping} and \ref{fig:mixture_after_mapping} show the scatter plots for each group of mixture distributions before and after matching.

For comparison, Figure \ref{fig:kmeans_plot} is  the results for the K-means matching with $k=3$ for samples generated from $X_0$ and $X_1$.   
The excellent performance of the proposed method can already be appreciated in this simple setting by comparing Figures \ref{fig:scatter_after_mapping} and \ref{fig:kmeans_scatter_after} as well as \ref{fig:ellipse_after} and \ref{fig:kmeans_ellipse_after}: the proposed method seems to obtain closer matches on average. Moreover, in areas where the overlap is somewhat worse the $3$-nearest neighbor approach does not provide matches at all, which is the case for instance in the north-east corner of Figure \ref{fig:kmeans_scatter_after}. By contrast, our proposed method provides good matchings for these individuals. The reason is that our proposed method matches all existing individuals without dropping observations. Optimal transportation is especially useful for this, as it can match distributions with different supports, in contrast to methods based on other divergences or distances. 

\subsection{Matching full Lalonde data set}

\begin{table}[htb]
	\setlength{\tabcolsep}{4pt}
	\centering
	\setlength\cmidrulewidth{0.15ex}
	\caption{Summary statistics and p-values to compare the $T_0$ sample and $T_1$ sample. t-test is used for the mean comparison, p-values denoted as $p_t$. F-test is used for the variance ratio comparison, p-values denoted as $p_F$. Kolmogorov–Smirnov test is used for testing the difference in the empirical CDF of two samples, p-values denoted as $p_{KS}$.}
	\begin{subtable}[t]{\columnwidth}
	\label{tb:lalonde_penalized}
	\caption{Penalized optimal transport, $\epsilon=10^{-3}$. Both \texttt{age} and \texttt{educ} are standardized. The matched covariates for \texttt{educ, black, hisp, married, nodegr} are rounded to the nearest integer.}
	\resizebox{0.5\columnwidth}{!}{%
	\begin{tabular}{lllllll}
        \multicolumn{7}{c}{Before matching}                                                                                                     \\
        \textbf{} & \textbf{x0.mean} & \textbf{x1.mean} & \textbf{t.p\_value} & \textbf{var.ratio} & \textbf{F.p\_value} & \textbf{KS.p\_value} \\
        age\_std  & -0.0111          & 0.0159           & 0.7216              & 0.9715             & 0.7820              & 0.8558               \\
        edu\_std  & -0.0464          & 0.0664           & 0.1443              & 0.7930             & 0.0291              & 0.1748               \\
        black     & 0.8000           & 0.8013           & 0.9645              & 1.0041             & 0.9749              & 1.0000               \\
        hispanic  & 0.1129           & 0.0943           & 0.4155              & 1.1721             & 0.1423              & 1.0000               \\
        married   & 0.1576           & 0.1684           & 0.7028              & 0.9475             & 0.6100              & 1.0000               \\
        nodegree  & 0.8141           & 0.7306           & 0.0092              & 0.7682             & 0.0130              & 0.1748               \\
        re75\_std & -0.0032          & 0.0046           & 0.9172              & 1.1384             & 0.2310              & 0.7938               \\
        \multicolumn{7}{c}{After OT matching ($\epsilon$ = $10^{-3}$)}                                                                          \\
        \textbf{} & \textbf{x0.mean} & \textbf{x1.mean} & \textbf{t.p\_value} & \textbf{var.ratio} & \textbf{F.p\_value} & \textbf{KS.p\_value} \\
        age\_std  & -0.0111          & -0.0111          & 1.0000              & 1.0688             & 0.5395              & 0.0421               \\
        edu\_std  & -0.0464          & -0.0464          & 1.0000              & 1.0748             & 0.5058              & 0.0000               \\
        re75\_std & 0.8000           & 0.7912           & 0.7748              & 0.9677             & 0.7542              & 1.0000               \\
        black     & 0.1129           & 0.1077           & 0.8264              & 1.0411             & 0.7124              & 1.0000               \\
        hispanic  & 0.1576           & 0.1549           & 0.9199              & 1.0135             & 0.9056              & 1.0000               \\
        married   & 0.8141           & 0.8215           & 0.7991              & 1.0312             & 0.7797              & 1.0000               \\
        nodegree  & -0.0032          & -0.0032          & 1.0000              & 1.0683             & 0.5428              & 0.0000               \\
        \multicolumn{7}{c}{After KNN (k=3) matching}                                                                                            \\
        \textbf{} & \textbf{x0.mean} & \textbf{x1.mean} & \textbf{t.p\_value} & \textbf{var.ratio} & \textbf{F.p\_value} & \textbf{KS.p\_value} \\
        age\_std  & -0.0111          & -0.0498          & 0.5791              & 1.3176             & 0.0110              & 0.2130               \\
        edu\_std  & -0.0464          & 0.0842           & 0.0594              & 1.1418             & 0.2203              & 0.0661               \\
        black     & 0.8000           & 0.8126           & 0.6718              & 1.0759             & 0.4998              & 1.0000               \\
        hispanic  & 0.1129           & 0.0943           & 0.4155              & 1.1721             & 0.1423              & 1.0000               \\
        married   & 0.1576           & 0.1650           & 0.7897              & 1.0124             & 0.9133              & 1.0000               \\
        nodegree  & 0.8141           & 0.7363           & 0.0136              & 0.8065             & 0.0430              & 0.1162               \\
        re75\_std & -0.0032          & -0.0643          & 0.3802              & 1.5025             & 0.0002              & 0.0000               \\
        \multicolumn{7}{c}{Propensity score matching (no rounding)}                                                                                           \\
           \textbf{} & \textbf{x0.mean} & \textbf{x1.mean} & \textbf{t.p\_value} & \textbf{var.ratio} & \textbf{F.p\_value} & \textbf{KS.p\_value} \\
    age\_std       & 0.0018           & 0.0131           & 0.7020              & 0.8814             & 0.2347              & 0.9778               \\
    edu\_std & 0.0058           & 0.0572           & 0.1065              & 0.7493             & 0.0066              & 0.0401               \\
    black     & 0.3067           & 0.3148           & 0.5036              & 0.9450             & 0.5924              & 0.0266               \\
    hispanic  & 0.0392           & 0.0329           & 0.4334              & 1.1516             & 0.1921              & 0.9396               \\
    married   & 0.0628           & 0.0684           & 0.6222              & 0.9087             & 0.3671              & 0.9273               \\
    nodegree  & 0.2944           & 0.2650           & 0.0115              & 0.7648             & 0.0116              & 0.0422               \\
    re75\_std      & 0.0030           & 0.0003           & 0.9270              & 1.1862             & 0.1147              & 0.4403           \\
            \multicolumn{7}{c}{Monge solution}                                                                                                      \\
                   \textbf{} & \textbf{x0.mean} & \textbf{x1.mean} & \textbf{t.p\_value} & \textbf{var.ratio} & \textbf{F.p\_value} & \textbf{KS.p\_value} \\
        age\_std  & -0.0111          & -0.0111          & 1.0000              & 1.0376             & 0.7357              & 0.4879               \\
        edu\_std  & -0.0464          & -0.0464          & 1.0000              & 1.0454             & 0.6836              & 0.3933               \\
        black     & 0.8000           & 0.7912           & 0.7748              & 0.9677             & 0.7542              & 1.0000               \\
        hispanic  & 0.1129           & 0.1145           & 0.9491              & 0.9873             & 0.8999              & 1.0000               \\
        married   & 0.1576           & 0.1549           & 0.9199              & 1.0135             & 0.9056              & 1.0000               \\
        nodegree  & 0.8141           & 0.8081           & 0.8389              & 0.9748             & 0.8067              & 1.0000               \\
        re75\_std & -0.0032          & -0.0032          & 1.0000              & 1.0422             & 0.7050              & 0.0058         
        \end{tabular}
	}
	\end{subtable}
% 	\begin{subtable}[t]{\columnwidth}
% 	\label{tb:lalonde_monge}
% 	\caption{Classical optimal transport without penalty. Only \texttt{age} is standardized. No rounding for the matched covariates.}
% 	\resizebox{\columnwidth}{!}{%
% 	\begin{tabular}{ l lll ll  l}
%  	\toprule
%  	    \multicolumn{6}{c}{Before Matching} \\
% 		 Covariates & $T_0$ mean & $T_1$ mean & $p_t$ & variance ratio & $p_F$ &$p_{KS}$\\
% 		 age & -0.0446 & 0.0627 & 0.2659 & 0.9730 & 0.8349 & 0.7481\\
%         educ & 10.0885 & 10.3459 & 0.1502 & 0.6446 & 0.0011 & 0.0629\\
%         black & 0.8269 & 0.8432 & 0.6474 & 1.0810 & 0.5742 & 1.0000\\
%         hisp & 0.1077 & 0.0595 & 0.0640 & 1.7156 & 0.0001 & 0.9630\\
%         married & 0.1538 & 0.1892 & 0.3342 & 0.8473 & 0.2200 & 0.9993\\
%         nodegr & 0.8346 & 0.7081 & 0.0020 & 0.6668 & 0.0027 & 0.0629\\
% 		\multicolumn{6}{c}{After OT Matching} \\
% 		Covariates & $T_0$ mean & $T_1$ mean & $p_t$ & variance ratio & $p_F$ &$p_{KS}$\\
% 		age & -0.0446 & -0.0446 & 1 & 1.0329 & 0.8189 & 0.9973\\
%         educ & 10.0885 & 10.0885 & 1 & 1.0262 & 0.8556 & 0.9332\\
%         black & 0.8269 & 0.8269 & 1 & 1.1168 & 0.4243 & 0.8409\\
%         hisp & 0.1077 & 0.1077 & 1 & 1.1791 & 0.2328 & 0.9861\\
%         married & 0.1538 & 0.1538 & 1 & 1.1029 & 0.4790 & 0.9939\\
%         nodegr & 0.8346 & 0.8346 & 1 & 1.1333 & 0.3653 & 0.8839\\
%         \multicolumn{6}{c}{After KNN Matching, $k=3$} \\
% 		Covariates & $T_0$ mean & $T_1$ mean & $p_t$ & variance ratio & $p_F$ &$p_{KS}$\\
% 		age & -0.0446 & -0.0136 & 0.7209 & 1.4377 & 0.0088 & 0.1507\\
%         educ & 10.0885 & 10.3802 & 0.0612 & 0.9975 & 0.9793 & 0.0629\\
%         black & 0.8269 & 0.8432 & 0.6474 & 1.0810 & 0.5742 & 1.0000\\
%         hisp & 0.1077 & 0.0595 & 0.0640 & 1.7156 & 0.0001 & 0.9630\\
%         married & 0.1538 & 0.1712 & 0.6250 & 0.9400 & 0.6443 & 1.0000\\
%         nodegr & 0.8346 & 0.7153 & 0.0033 & 0.6848 & 0.0051 & 0.0629\\
%  		\bottomrule
% 	\end{tabular}%
% 	}
% 	\end{subtable}
	\label{tb:lalonde}
\end{table}


==> yuliang/ATE_old.tex <==
\section{Causal effects via optimal transport matching}\label{sec:ATE}
This section connects the matching problem to inference on causal effects. We rely on the potential outcome framework \citep{imbens2015causal, rubin1974estimating}. Let $Y(j)$ be the potential outcome under the causal inference framework for treatment $j\in \{1,...,J\}$, $T$ be the treatment assignment, and random variable $D$ supported on $\{\tau\in \{0,1\}^J: \sum_{j=1}^J \tau_j=1\}$ be the binary vector of the treatment assignment: $T=j$ if and only if $D(j)=1$. $X\in\mathbb{R}^d$ is the vector of observed covariates. We make the following set of assumptions, the first three standard in the literature \citep{abadie2006large, imbens2000role, imbens2015causal}.
\begin{assumption}\label{ass:causal}
For $j=1,..,J$,
\begin{enumerate}
    \item (Weak unconfoundedness) $D(j) \independent Y(j)|X$,
    \item (Overlap) $P(D(j)=1|X)$ is bounded away from 0 and 1,
    \item Conditional on $D(j)=1$, the sample is independently drawn from $(Y,X)|D$, and the marginal $X\sim \mu_j$ given $D(j)=1$,
    \item Given $D(j)=1$, there exists a bounded continuous function $f_j$ supported on a convex and compact set $\mathcal{X}_j\subset \mathbb{R}^d$ such that $f_j(X) = \mathbb{E}(Y|T=j,X)$. For a more explicit notation, we use $y(j,X):=f_j(X)$ and $\varepsilon_i = Y_i-y(T_i,X_i)$ are i.i.d. mean-zero noise terms.
    % \item Given $D(j)=1$, there exists a bounded continuous function $f_j$ supported on a convex and compact set $\mathcal{X}_j\subset \mathbb{R}^d$ such that $Y(j)=f_j(X)+\epsilon$. For a more concise notation, we use $y(j,X):=f_j(X)$ and $Y(j, X):=f_j(X)+\epsilon$.
\end{enumerate}
\end{assumption}
Parts 1 and 2 of Assumption \ref{ass:causal} are standard. The weak unconfoundedness assumption formalizes the idea of matching on observables: it guarantees that there are no more systematic differences between the unobservable covariates of the groups once the observable characteristics have been accounted for. The weak unconfoundedness assumption was introduced in \citet{imbens2000role} and is slightly weaker than the strong unconfoundedness assumption introduced in \citet{rosenbaum1983central} since it is locally constrained for every realization of the treatment assignment. The overlap assumption guarantees that one can find appropriate matches in each group. If this were not the case, the estimate of the causal effect would be biased. It is a fundamental assumption for any matching approach \citep{imbens2015causal}. Part 3 of Assumption \ref{ass:causal} states that all treatment groups are independently sampled; a similar assumption is made in classical matching approaches \citep{abadie2006large}. Part 4 introduces regularity assumptions that are weaker than existing assumptions. In particular, we do not specify any parametric restrictions on the relationship between $Y$ and $X$ like linearity or convexity and only require additive separability analogously to \citet{abadie2006large}. 

Under part 3 in Assumption \ref{ass:causal}, we can denote $X_j := X|D(j)=1$, $X_j\sim \mu_j$ and $\gamma$ as the joint coupling over $\prod_{j=1}^J\mathcal{X}_j$ with the marginal distributions $(\mu_1,...,\mu_J)$ obtained via the proposed matching procedure. The expected counterfactual outcome $E[Y(t)]$ for treatment $T=t$ can then be written as $\mathbb{E}\{Y(t)\} = \mathbb{E}_{X}\left\{ \mathbb{E}(Y(t)|D(t)=1,X) \right\} = \mathbb{E}_X\{y(t,X)\}$.

In the population one hence knows the counterfactual outcome $Y(j)$ for any treatment status $T=j$. This is not the case in realized samples, however, which is the ``fundamental problem of causal inference'' \citep{holland1986statistics}: for each individual $i=1,\ldots, N$ the researcher only observes one potential outcome $Y_i(j)$ for the given treatment $T=j$ that the individual was assigned to. In order to compute the causal effect of a treatment, the researcher should compare $Y_i(j)$ to $Y_i(k)$, $k\neq j$ for each $i$, which is impossible. The idea of matching on covariates is hence to impute the counterfactual outcomes $Y_i(k)$ for individual $i$ by considering the outcomes of other individuals that received a different treatment $k$. The unconfoundedness assumption implies that individuals with similar observable covariates also possess similar unobservable characteristics, which makes matching on observable covariates a feasible approach. This implies that two individuals with the same observable covariates do not systematically differ in their heterogeneity and that one can consider the observed outcome of one individual as the potential outcome of another. This leads us to the following definition of the potential outcome imputed by our proposed method.

% \begin{definition}\label{def:matching_po1}
% Let $\gamma_{j|t}$ be the conditional distribution of covariates in group $T=j$ given covariates in group $T=t$, and $\hat\gamma_{N,j|t}$ be the finite sample version. Then the estimator for the average treatment effect of treatment $t$ compared to treatment $j$ can be defined as
% \begin{align*}
%     &\widehat{\mathbb{E} \{Y(t) - Y(j)\}} \\=& 
%     \frac{1}{N}\sum_{i=1}^{N}\left\{ Y_iI(D_i(t)=1) - \sum_{x_k\in\text{supp}(\hat\gamma(X_j|X_t))} Y_k\hat\gamma(X_j=x_k|X_t=x_i) I(D_i(j)=1) \right\}
% \end{align*}
% \end{definition}
% \[\sum_{k\neq i} Y_k \hat{\gamma}_{N,j|t}(X_k|X_i)I(D_i(t)=1) \]


\begin{definition}\label{def:matching_po1}
For the $j$-th treatment and $t\neq j$ denote $\gamma_{j|t}$ as the conditional measure of covariates in group $j$ given the covariates in group $t$ under the joint distribution $\gamma$. 
Then under Assumption \ref{ass:causal}, the expected potential outcome can be expressed in the sample version as
% \begin{equation}
% \begin{aligned}
%     \mathbb{E}\{Y(j)\}&= \mathbb{E}_{X}\left( y(T,X)I(D(j)=1) \right) + \mathbb{E}_{X}\left( y(T,X)I(D(j)=0) \right)
%     \\
%     &=\int_{\mathcal{X}_j} y(j,x) \dd\mu_j(x) + \int_{\mathcal{X}_j} \sum_{t\neq j}\int_{\mathcal{X}_{t}  } y(t,x) \dd\gamma(x_t|x_j) \dd\mu_j(x_j) \label{eq:po_pair}
% \end{aligned}
% \end{equation}
% The corresponding sample version is 
\begin{equation}\label{eq:sample_po}
    \widehat{\mathbb{E} \{Y(j)\}} = \frac{1}{N}\sum_{i=1}^N Y_i I(D_i(j)=1) + 
    \frac{1}{N}\sum_{i=1}^N \sum_{t\neq j} \sum_{k\neq i} Y_k \hat{\gamma}_{N,j|t}(X_k|X_i)I(D_i(t)=1),
\end{equation}
where $N = \sum_{j=1}^J N_j$ is the overall number of sample points over all treatment arms and $\hat{\gamma}_N$ is the empirical counterpart to the optimal matching estimated via the IPFP \eqref{eq:sinkhornconv} by replacing $\mu_j$ with the empirical measures $\hat{\mu}_{N_j}$ defined below in \eqref{eq:empmeas}.
\end{definition}
Definition \ref{def:matching_po1} focuses on the expected potential outcome, but the formulation \eqref{eq:sample_po} provides a general way to obtain estimators of many different types of causal effects: average treatment effects can be obtained as a difference of expected potential outcomes; quantile treatment effects or differences in Gini coefficients \citep[chapter 20]{imbens2015causal} can be obtained by composing $Y_i$ with different functions. It is also straightforward to obtain conditional causal effects by conditioning on specific covariate values $X=x$.

For comparison, recall that the $k$-nearest neighbors matching estimator for the potential outcome $Y_i(0)$ in the binary treatment case in \cite{abadie2006large} is defined as 
\begin{equation}\label{eq:kmeans_po}
    \hat Y_i(0) = \begin{cases} Y_i, & \text{if } T_i=0,\\
\frac{1}{M}\sum_{j\in\mathcal{J}_M(i)}Y_j, & \text{if } T_i=1
\end{cases}
\end{equation}
where $\mathcal{J}_M(i)$ is a group of M matches that are closest to $i$. This group is determined by the distance between the covariates $X_j$ and $X_i$. In analogy to (\ref{eq:kmeans_po}) we can write (\ref{eq:sample_po}) as

\begin{equation}\label{eq:sample_po2}
    \hat Y_i(0) = \begin{cases} Y_i, & \text{if } T_i=0,\\
\sum_{k\neq i} Y_k \hat{\gamma}_{N,0|t}(X_k|X_i)I(D_i(t)=1), & \text{if } T_i=t,t\neq 0
\end{cases}
\end{equation}


The estimator of the expected counterfactual outcome proposed in (\ref{eq:sample_po}) is analogous to the $k$-nearest neighbor idea (\ref{eq:kmeans_po}), with $\mathcal{J}_M(i)$ being replaced by the support of $\hat\gamma_{N,j|t}$, and the equal weight $\frac{1}{M}$ replaced by the probability mass $\hat\gamma_{N,0|t}(X_k|X_i)$. Moreover, recall that in the binary treatment setting, the propensity score approach uses the Horvitz-Thompson type estimator \citep{horvitz1952generalization} with the selection probability $r(t,x) := \mathbb{P}(T=t|X=x)$ to estimate the average treatment effect $\mathbb{E}(Y(t)) = \mathbb{E} \left(\frac{YI(T=t)}{r(t,X)}\right)$, or alternatively $\mathbb{E}\left\{\mathbb{E}(Y(t)|r(t,X))\right\}$, which shows the connection of the proposed method \eqref{eq:sample_po} to the propensity score approach.
% \yxcm{Maybe add something here to explain why HT estimator is not used?}

%As discussed in \cite{imbens2000role}, one limitation of the propensity score approach lies in extending this idea to the multiple treatment case. Recent development such as \cite{li2019propensity} provide different weightings for balancing on the covariates under multiple treatments. However, these weights are usually difficult to interpret, and the balancing effect strongly depends on the correctly specified propensity score model. In Definition \ref{def:matching_po1}, using the interpretable conditional probability $\gamma_{j|t}$ as the weight, the balancing is automatically obtained since $\gamma_{j|t}$ is the optimal transport that maps $\mu_j$ to $\mu_t$. The term $\sum_{k\neq i} Y_k \hat{\gamma}_{N,j|t}(X_k|X_i)I(D_i(t)=1)$ is the finite sample analogue to the population version $\int_{\mathcal{X}_j}Y(j,x)\dd\gamma_{j|t}(x|x_i)$, which can be interpreted as the potential outcome $Y(j)$ given $X_t$ if the group $X_t$ had been assigned treatment $j$. 

%Definition \ref{def:matching_po1} estimates the average treatment effect based on matchings from $\mu_j$ to all other marginals $\mu_{[-j]}$. This joint approach can be costly in high dimensional settings with many treatments. Alternatively, we could also match all marginals to a barycenter, as mentioned. In this case we have the following definition for the expected potential outcome.
%\begin{definition}\label{def:matching_bc}
%Let $\mu_b$ be the barycenter distribution. Denote $\gamma_{j|b}$ as the conditional matching for covariates in group $j$ and the barycenter, under the joint distribution $\gamma$. 
%Then under Assumption \ref{ass:causal}, the expected potential outcome for the treatment $j$ conditioning on the barycenter group $X_b$ can be defined as follows,
%\begin{align}
    %\mathbb{E}\{Y(j)|X_b\}&= 
    %\int_{\mathcal{X}_{j} } y(j,x) \dd\gamma_{j|b}(x|x_b) \label{eq:bc_pair}
%\end{align}
%The corresponding sample version is 
%\begin{equation}\label{eq:sample_bc}
    %\widehat{\mathbb{E} \{Y(j)|X_b\}} =
   % \sum_{X_k\in\text{supp}(\hat\gamma_{N,j|b})} Y_k \hat\gamma_{N,j|b}(X_k|X_b)
%\end{equation}

%\end{definition}
% Definition \ref{def:matching_bc} can be modified to condition on any other treatment $t$ instead of the barycenter, by replacing $\gamma_{j|b}$ by $\gamma_{j|t}$. In practice, the matching between $X_j$ and $X_t$ can be obtained from the two pairwise joint distributions $\gamma(x_j,x_b)$ and $\gamma(x_t,x_b)$, with a further step $\mathbb{E}_{X_b} \{ \mathbb{E}\{Y(j)|X_b\}|X_t\}$. For example, if we denote $M_j$ as the discrete joint distribution of $(X_j,X_b)$ such that $X_bM_j\sim \hat\mu_j,X_jM_j^T\sim\hat\mu_b$, and $M_t$ as the joint distribution of $(X_t,X_b)$, where $X_bM_t\sim \hat\mu_t,X_tM_t^T\sim\hat\mu_b$, then $M_{t,j}:=M_t^T M_j$ is the joint distribution of $(X_j,X_t)$ under the pairwise joint matching $\hat\gamma$ such that $X_tM_{t,j}\sim\hat\mu_j$ and $X_jM_{t,j}^T\sim\hat\mu_t$. In this way, we only need to know the $J$ matchings from each marginals to the barycenter, to recover all $\binom{J}{2}$ pairwise matchings. Definition \ref{def:matching_bc} also provides a way to directly compare the treatment effect $\mathbb{E}(Y(j)|X_t )-\mathbb{E}(Y(t)|X_t )$.
 
%  In fact, if the strong unconfoundedness assumption is available, i.e. $Y\independent D|X$ instead of $Y(j)\independent D(j)|X$, which means $Y(j)\independent D(t)|X$ even when $t\neq j$, then we could obtain $\mathbb{E}(Y(j)|X_t)$ when $j\neq t$ using the optimal transport matching $\gamma(x_j,x_t)$,
%  \begin{align*}
%      \mathbb{E}(Y(j)|X ) &= \mathbb{E}(Y(j)|X, T=t ) =\mathbb{E}(Y(j)|X_t ) \\ &=  
%      \mathbb{E}_{X_j} \left\{ \mathbb{E}(Y(j)| X_j,X_t)\right\} = \mathbb{E}_{X_j} \left\{ \mathbb{E}(Y(j)| X_j)|X_t\right\} = \int_{\mathcal{X}_j} \mathbb{E}(Y(j)| X_j) \dd\gamma(x_j|x_t)
%  \end{align*}
% In this way, we could directly compare $\mathbb{E}(Y(j)|X_t )-\mathbb{E}(Y(t)|X_t )$, since they are both measurable functions on $\sigma(\mathcal{X}_t)$. Note that with the weak unconfoundedness assumption, this is not true, because $\mathbb{E}(Y(j)|X_t) \neq \mathbb{E}(Y(j)|X,T=t )$ since given $X$, $Y(j)$ and $D(t)$ are no longer independent.
% \yxcm{Todo: 1.add comparison; 2. add a corollary for the conditional distribution after theorem 1. }




==> yuliang/Proof_of_lemma1.tex <==
\begin{proof}[Proof of Theorem \ref{thm:potential}]
We prove the statement using standard results from empirical process theory \citep{wellner2013weak, kosorok2008introduction}, in particular results for $Z$-estimators. We consider the integrated version of the Schr\"odinger system \eqref{eq:FOC} a $Z$-estimator in the sense of Theorem 3.3.1 in \citet{wellner2013weak} and Theorem 13.4 in \citet{kosorok2008introduction}. In particular, the first-order equations \eqref{eq:FOC} are derived by requiring that the first variation $\delta F(\varphi^*,v)$ \citep[Definition 40.2]{zeidler2013nonlinear} of the objective function \eqref{eq:dual} in any direction $v\in \prod_{j=1}^JL^1(\mu_j)$ vanishes at the optimal $\varphi^*$, i.e.
\begin{equation}\label{eq:firstvariation}
\begin{aligned}
0=\delta F(\varphi^*,v)\coloneqq&\int_{\mathcal{X}}\sum_{j=1}^Jv_j\left[\exp\left(\frac{\sum_{j=1}^J\varphi^*_j - c}{\varepsilon}\right)-1\right]\dd\bigotimes_{j}\mu_j\\
=&\sum_{j=1}^J\int_{\mathcal{X}_j}v_j\int_{\mathcal{X}_{-j}}\left[\exp\left(\frac{\sum_{j=1}^J\varphi^*_j - c}{\varepsilon}\right)-1\right]\dd\bigotimes_{i\neq j}\mu_i\dd\mu_j,\\
\end{aligned}
\end{equation}
where the last line follows from Fubini's theorem and the boundedness of all integrands. \eqref{eq:firstvariation} holds if and only if the first order conditions \eqref{eq:FOC} are satisfied. We consider  $v\in \prod_j L^1(\mu_j)$ because $\sum_jv_j$ and the term in brackets in \eqref{eq:firstvariation} form a natural duality bracket in $\left(\prod_jL^1(\mu_j),\prod_jL^\infty(\mu_j)\right)$, i.e.~the G\^ateaux derivative
\[F'(\varphi)\coloneqq \exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right)-1\in \left(\prod_jL^1(\mu_j)\right)^* = \prod_jL^\infty(\mu_j)\] satisfies
\[\delta F(\varphi,v) = \left\langle F'(\varphi),\sum_jv_j\right\rangle,\] see \citet[section 40.1]{zeidler2013nonlinear}. By Fubini's theorem we can also write the first variation in terms of the Schr\"odinger equations \eqref{eq:FOC} as
\[\delta F(\varphi,v) = \sum_{j=1}^J\left\langle T_j(\varphi)-1,v_j\right\rangle_j,\] where
\[T_j(\varphi)(x_j) = \int_{\mathcal{X}_{-j}}\exp\left(\frac{\sum_j\varphi_j(x_j)-c(x)}{\varepsilon}\right)\dd\bigotimes_{i\neq j}\mu_i(x_{-j})\] and $\langle\cdot,\cdot\rangle_j$ is the duality bracket with respect to $\mu_j$.

We can now focus on proving the lemma. It will be based on Theorem 3.3.1 in \citet{wellner2013weak} and Theorem 13.4 in \citet{kosorok2008introduction}. We need to show the following:
\begin{itemize}
    \item[(i)] $\left\|\hat{\varphi}_N-\varphi^*\right\|_{L^\infty} = o_P(1)$
    \item[(ii)] There exists some $\delta>0$ such that the classes
    \begin{multline*}\tilde{\mathcal{F}}_{\delta}\coloneqq\left\{\sum_{j=1}^J v_j\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right)- 1\right]: \|\varphi - \varphi^*\|_{C^k}<\delta\thickspace \forall k\in\mathbb{N}^d_0,\right.\\ \left. \thickspace v\in B_1\left(\prod_{j=1}^J C^\infty_c(\mathcal{X}_j)\right), \varphi\in \prod_jC^\infty(\mathcal{X}_j)\right\}
    \end{multline*} are $\bigotimes_j\mu_j$-Donsker (see chapters 2.1 and 2.5 in \citet{wellner2013weak} for a definition of Donsker classes). Here, $C^\infty_c(\mathcal{X}_j)$ is the space of all smooth functions with compact support on $\mathcal{X}_j$ and $B_1\left( C^\infty_c(\mathcal{X}_j)\right)$ is the unit ball in $C_c^\infty(\mathcal{X}_j)$, i.e.~the set of all functions $v_j$ with $\|v_j\|_{C^k(\mathcal{X}_j)}\leq 1$ for any multi-index $k\in\mathbb{N}^d_0$.
    \item[(iii)] As $\|\varphi-\varphi^*\|_{L^\infty}\to0$
    \[\sup_{v_j\in B(C_c^\infty(\mathcal{X}_j))}\int_{ \mathcal{X}}\left\{\sum_{j=1}^J v_j\right\}^2\left(\exp\left(\frac{\sum_j\varphi_j-c}{\varepsilon}\right) - \exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon}\right)\right)^2\dd\bigotimes_{ j}\mu_j\to0,\quad\text{$j=1,\ldots, J$}\]
    \item[(iv)] 
    $\Psi(\varphi^*) = \int_{\mathcal{X}}\left[\exp\left(\frac{\sum_{j=1}^J\varphi^*_j - c}{\varepsilon}\right)-1\right]\dd\bigotimes_{j}\mu_j$
    % $\delta F(\varphi, v)$ 
    % $T(\varphi)\coloneqq (T_1(\varphi),\ldots, T_J(\varphi))$ 
    is Fr\'echet-differentiable with continuously invertible derivative 
    \[ \dot{\Psi}(\varphi^*)(u) = \frac{1}{\varepsilon}\int_{\mathcal{X}}\exp\left(\frac{\sum_{j=1}^J\varphi_j^*-c}{\varepsilon}\right)\sum_{j=1}^Ju_j\dd\bigotimes_{j}\mu_j\] 
    at $\varphi^*$ for all $u\coloneqq (u_1,\ldots,u_J)\in\prod_{j=1}^J L^\infty(\mu_j)$. 
    \item[(v)] Denote $\Psi_N(\varphi):=\int_{\mathcal{X}}\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right)-1\right]\dd\bigotimes_{j}\hat\mu_j$.
    \[\Psi_N(\hat\varphi_N) = o_P(N^{-1/2})\] for $\hat{\varphi}_N\in F$.
    
    % Use the empirical process notation $\mathbb{P}_Nf:=\int_{\mathcal{X}}f(x)\dd\bigotimes_{j}\hat\mu_j(x)$. $\delta F(\varphi,v)$ can be seen as an operator on $v$ indexed by $\varphi$, 
    
    
    % and 
    % \[P\left( \left\|\left(\sqrt{N_1}\hat{T}_{N_1}^b(\hat{\varphi}^b_{N}), \ldots, \sqrt{N}_J \hat{T}_{N_J}^b(\hat{\varphi}^b_{N})\right)\right\|_{L^\infty}>\eta\rvert \mathbb{X}_N\right)=o_P(1),\]
    % where $\mathbb{X}_N$ denotes the sample drawn and where $\hat{T}^b_N(\hat{\varphi}^b_N)$ denotes a bootstrapped version of the operator \citep[Theorem 13.4]{kosorok2008introduction}, i.e.~where we estimate the measures $\mu_j$ via some (multiplier) bootstrap procedure, see \citet[section 3.6]{wellner2013weak} for details on the bootstrap. 
\end{itemize}
We prove each requirement one by one before putting everything together.\\

\noindent\emph{Requirement (i):}
This follows from Lemma \ref{lem:consistency}. \\

\noindent\emph{Requirement (ii):} 
This requirement is needed to provide the asymptotic equicontinuity of the empirical process map corresponding to the estimation equation 
\[\delta F(\varphi^*,v) =0\quad\text{for all $v\in  B_1\left(\prod_jC^\infty_c(\mathcal{X}_j)\right)$},\] where $B_1\left(\prod_jC^\infty_c(\mathcal{X}_j)\right)$ denotes the unit ball of all smooth functions $v\equiv (v_1,\ldots, v_J)$ with compact support on $\prod_j\mathcal{X}_j$.\footnote{The space of smooth functions is a Fr\'echet space, so a general way to consider the unit ball in this Fr\'echet space is to define a weighted series of the $C^k$-norms that makes the ``$C^\infty$-norm'' summable, see \citet{treves2006topological} for details.} The weak convergence of the empirical process of the first-order condition required for obtaining the asymptotic distribution of the empirical process of the potentials can then be shown by the weak convergence of the empirical process corresponding to the first variation \eqref{eq:firstvariation} for all $v$ in a sufficient index set $\mathcal{S}\subset \prod_{j=1}^JL^1(\mu_j)$ by Lemma 3.3.5 in \citet{wellner2013weak}. A sufficient condition that also provides the fact that this asymptotic distribution will be a tight mean-zero Gaussian process is exactly requirement (ii) above for $\mathcal{S}= B_1\left(\prod_j C^\infty_c(\mathcal{X}_j)\right)$ and follows from Theorem 13.4 (C) in \citet{kosorok2008introduction}. 

So to show requirement (ii) we hence have to show two things. First, we need to show that we can set $\mathcal{S}\coloneqq B_1\left(\prod_jC^\infty_c(\mathcal{X}_j)\right)$. Second, we need to show that $ \mathcal{\tilde F}_{\delta}$ is indeed $\bigotimes_j\mu_j$-Donsker. For the first statement note that
\begin{equation}\label{eq:boundexp}
\begin{aligned}
&\left\lvert\exp\left(\frac{\sum_j\varphi_j-c}{\varepsilon}\right)-\exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon}\right)\right\rvert\\
=&\left\lvert\exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon}\right)\left[\exp\left(\frac{\sum_j\varphi_j-\varphi^*_j}{\varepsilon}\right)-1\right]\right\rvert\\
\leq & \exp\left(\frac{\sum_j\left\|\varphi^*_j\right\|_{L^\infty}(\mu_j)-c}{\varepsilon}\right)\left\lvert\exp\left(\frac{\sum_j\varphi_j-\varphi^*_j}{\varepsilon}\right)-1\right\rvert\\
&\leq \exp\left(\frac{\sum_j\left\|\varphi^*_j\right\|_{L^\infty(\mu_j)}-c}{\varepsilon}\right)\left\lvert\exp\left(\frac{\sum_j\left\|\varphi_j-\varphi^*_j\right\|_{L^\infty(\mu_j)}}{\varepsilon}\right)-1\right\rvert.
\end{aligned}
\end{equation}
which shows that this term is continuous in some $\prod_j L^\infty(\mu_j)$-neighborhood of $\varphi^*$.
Taking the supremum over $\prod_{j=1}^J\mathcal{X}_j$ on both sides of the inequality while noting that $c(x_1,\ldots,x_J)\geq0$
implies
\begin{multline*}
\left\|\exp\left(\frac{\sum_j\varphi_j-c}{\varepsilon}\right)-\exp\left(\frac{\sum_j\varphi^*_j-c}{\varepsilon}\right)\right\|_{L^\infty}\\\leq \exp\left(\frac{\sum_j\left\|\varphi^*_j\right\|_{L^\infty(\mu_j)}}{\varepsilon}\right)\left\lvert\exp\left(\frac{\sum_j\left\|\varphi_j-\varphi^*_j\right\|_{L^\infty(\mu_j)}}{\varepsilon}\right)-1\right\rvert,
\end{multline*}
which vanishes as $\sum_j\|\varphi_j-\varphi^*_j\|_{L^\infty(\mu_j)}\to0$. Therefore, the G\^ateaux- derivative obtained via the first variation \eqref{eq:firstvariation} coincides with the Fr\'echet-derivative \citep[p.~192]{zeidler2013nonlinear}. Now Fr\'echet differentiability in particular implies that the convergence of the linear approximation to the derivative at $\varphi^*$ from any direction $v\in\prod_jL^1(\mu_j)$ is of the same rate. This further implies that we can infer the derivative in any direction $v\in \prod_j L^1(\mu_j)$ by only considering directions in a dense subset of $\prod_j L^1(\mu_j)$. In particular, the equality \eqref{eq:firstvariation} only has to hold for all $v$ in a dense subset of the unit ball of $\prod_{j=1}^JL^1(\mu_j)$. But $\prod_{j=1}^J C_c^\infty(\mathcal{X}_j)$ is dense in $\prod_{j=1}^J L^1(\mu_j)$ \citep[Proposition 8.17]{folland1999real}, so that we can focus on the unit ball in $\prod_j C_c^\infty(\mathcal{X}_j)$.  

So now we need to show that there exists some $\delta>0$ such that $\mathcal{\tilde F}_{\delta}$ is $\bigotimes_j\mu_j$-Donsker. For this, we use the concept of bracketing entropy and bracketing numbers \citep[chapter 2.7]{wellner2013weak}. Since $\prod_jL^\infty(\mu_j)$ is a Banach lattice under the standard ordering $f\preceq g \Leftrightarrow f_j(x_j)\leq g_j(x_j)$ for $\mu_j$-almost all $x_j$ and all $j$, we can define, for any two functions $f_l, f_u\in \prod_j L^\infty(\mu_j)$ the bracket $[f_l,f_u]$ as the set of all functions $f$ such that $f_l\preceq f\preceq f_u$. A $\eta$-bracket is a bracket $[f_l,f_u]$ with $\|f_u-f_l\|_{L^\infty}<\eta$. For some set $\mathcal{F}$ of functions the bracketing number $N_{[\medspace]}\left(\eta,\mathcal{F},\|\cdot\|\right)$ is the minimum number of $\eta$-brackets needed to cover $\mathcal{F}$ in the metric induced by $\|\cdot\|$ \citep[p.~83]{wellner2013weak}. 

To show that $\mathcal{F}_\delta$ is $\bigotimes_j\mu_j$-Donsker for some $\delta>0$ we want to show that the corresponding bracketing entropy integral is finite, i.e.~that
\begin{equation}\label{eq:entropyint}
\int_0^\infty \sqrt{\ln N_{[\thinspace]}\left(\eta,\mathcal{F}_\delta, L^2(\bigotimes_{j}\mu_j)\right)}d\eta<+\infty.
\end{equation}
The idea is to treat $\sum_j v_j$ and 
\[g_\varphi(x_1,\ldots,x_J) \equiv g_\varphi(x) \coloneqq \exp\left(\frac{\sum_{j=1}^J\varphi_j(x_j) - c(x)}{\varepsilon}\right)-1\] separately.
The reason is that Corollary 2.7.2 in \citet{wellner2013weak} in combination with the fact that $\mathcal{X}_j\subset\mathbb{R}^d$ is compact implies that $B_1(\prod_jC_c^\infty(\mathcal{X}_j))$ is $\bigotimes_j\mu_j$-Donsker for any dimension $d$. Moreover, it is a uniformly bounded set. If we can show that the set of all functions $g_\varphi$ for some $\delta>0$ is also a uniformly bounded Donsker class for any dimension $d$, then their product, i.e.~$\mathcal{F}_\delta$, will be a Donsker class for any dimension by Example 2.10.8 in \citet{wellner2013weak}. 

Now by Lemma \ref{lem:varphiopt} the optimal $\varphi^*$ obtained via the Sinkhorn algorithm is smooth. Since this holds for any set of measures $\{\mu_j\}_{1\leq j\leq J}$ it also holds for $\hat{\varphi}_n$. Moreover, by Lemma \ref{lem:consistency} we know that $\hat{\varphi}_{N_j}$ converges to $\varphi^*_j$ in $C^\infty(\mathcal{X}_j)$. Hence for some small $\delta>0$ we can find a uniform bound for the $\hat{\varphi}_{N_j}$ in $C^\infty(\mathcal{X}_j)$ by the reverse triangle inequality:
\[\left\lvert \left\|\hat{\varphi}_N\right\|_{C^k} - \left\|\varphi^*\right\|_{C^k}\right\rvert\leq \left\|\hat{\varphi}_N-\varphi^*\right\|_{C^k}<\delta,\] for some $\delta>0$ and all multi-indices $k\in\mathbb{N}_0^d$. 

We can now show that the classes 
\begin{multline*}\tilde{\mathcal{F}}_{\delta}\coloneqq\left\{\sum_j v_j\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right)- 1\right]: \|\varphi - \varphi^*\|_{C^k}<\delta\thickspace \forall k\in\mathbb{N}_0^d\right.,\\ \left.\thickspace v\in B_1\left(\prod_{j} C^\infty_c(\mathcal{X}_j)\right), \varphi\in \prod_jC^\infty(\mathcal{X}_j)\right\}
\end{multline*}
are Donsker.
In fact, the class
\[\mathcal{G}_{\delta}\coloneqq\left\{\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right)- 1\right]: \|\varphi - \varphi^*\|_{C^k}<\delta\thickspace\forall k\in\mathbb{N}_0^d, \varphi\in \prod_jC^\infty(\mathcal{X}_j)\right\}\] is a bounded subset of $\prod_j C^\infty(\mathcal{X}_j)$ for compact and convex $\mathcal{X}_j$. Therefore by Corollary 2.7.2 $\mathcal{G}$ is a uniformly bounded Donsker class for any dimension $d$. This implies by Example 2.10.8 in \citet{wellner2013weak} that $\tilde{\mathcal{F}}_{\delta}$ is a $\bigotimes_j\mu_j$-Donsker class in any dimension $d$.\\

\noindent\emph{Requirement (iii):} 
This follows immediately by the fact that all $\mathcal{X}_j$ are compact and an analogous bound to \eqref{eq:boundexp}. \\

\noindent\emph{Requirement (iv):}
\yxcm{Proposition 4.1 shows injective map.}


This follows from Proposition 3.1 in \citet{carlier2020differential}, which shows that $T'(\varphi)$ is an isomoprhism between $G$ and $H$. In particular, by the inverse function theorem in Banach spaces, $T'(\varphi)$ is a local $C^\infty$-diffeomorphism between $E$ and $F$. Moreover $T(G)$ is open in $H_{++}$.\\

\noindent\emph{Requirement (v):}
This follows from the linear convergence of the IPFP/Sinkhorn iterations as shown in \citet{carlier2021linear}. In particular, Remark 3.4 in \citet{carlier2021linear} implies that there for any $N$ there exists some $m\in\mathbb{N}$ such that both criteria are satisfied. As mentioned in the main text this $m$ can be rather large because of the exponential bound proved in Theorem 3.3 in \citet{carlier2021linear}. \\

We can now put everything together by using Theorem 3.3.1 in \citet{wellner2013weak} and Theorem 13.4 in \citet{kosorok2008introduction}. We show that the five requirements above imply the requirements (A) to (F) in Theorem 13.4 in \citet{kosorok2008introduction}. (A) is implied by the fact that the optimum $\varphi^*$ is well-separated, which in turn follows from the fat that $T(\varphi)$ is strictly convex in $\varphi$. (B) is implied by (i). (C) is implied by (ii). (D) is implied by (iii). (E) is implied by (v). Finally, (F) is implied by (iv). Hence Theorem 13.4 in \citet{kosorok2008introduction} implies that
\[\left(\sqrt{N_1}\left(\hat{\varphi}_{N_1} - \varphi_1^*\right),\ldots, \sqrt{N_J}\left(\hat{\varphi}_{N_J}-\varphi_J^*\right)\right) \rightsquigarrow - \left(T'(\varphi^*)\right)^{-1}(Z),\] 
where $Z$ is the tight mean-zero Gaussian limit process of 
\[\left(\sqrt{N_1} \left(\hat{T}_{N_1}(\varphi^*) - T_1(\varphi^*)\right),\ldots, \sqrt{N_J} \left(\hat{T}_{N_J}(\varphi^*) - T_J(\varphi^*)\right)\right)\]
in the space $\ell^\infty\left(\prod_j L^\infty(\mu_j)\right)$ of bounded functions on $\prod_jL^\infty(\mu_j)$. Moreover, Theorem 13.4 in \citet{kosorok2008introduction} directly implies that a standard bootstrap procedure is valid.
\end{proof}

==> yuliang/Proof_of_lemma3.tex <==

\newcommand{\K}{\mathcal{K}}
\begin{proof}
Just as in the proof of Proposition 1 in \cite{genevay2019sample} we consider the univariate setting, i.e.~where each $x_j\in\mathbb{R}$. The extension to the multivariate setting is straightforward.
By rearranging terms in (\ref{eq:FOC}), we get
\[
    \exp\left(-\frac{\varphi_j(x_j)}{\varepsilon}\right)
    =\int_{\mathcal{X}_{-j}} \exp\left(\frac{\sum_{i\neq j}\varphi_i(x_i) - c(x_1,\ldots,x_J)}{\varepsilon}\right)\dd\bigotimes_{i\neq j}\mu_i(x_{-j})
\]
After taking the first derivative on both sides and rearranging,
\[
    \varphi_j'(x_j)
    =\int_{\mathcal{X}_{-j}} \exp\left(\frac{\sum_{i}\varphi_i(x_i) - c(x_1,\ldots,x_J)}{\varepsilon}\right) \frac{\partial c(x_1,...,x_J)}{\partial x_j} \dd\bigotimes_{i\neq j}\mu_i(x_{-j})
\]

Denote $\K_\varepsilon(x): = \exp\left(\frac{\sum_{i}\varphi_i(x_i) - c(x_1,\ldots,x_J)}{\varepsilon}\right)$, and $c'_j(x) =\frac{\partial c(x)}{\partial x_j}$. 
Note that 
\[\frac{\partial}{\partial x_j} \K_\varepsilon(x) = \K_\varepsilon(x)\frac{ \varphi'_j(x_j)- c'_1(x)}{\varepsilon}.\] The $n$-th order derivative of the potentials can be obtained by recurrence,
\begin{align*}
    \varphi_j^{(n)}(x_j) &= \int_{\mathcal{X}_{-j}} \K_\varepsilon(x) g_n(x) \dd\bigotimes_{i\neq j}\mu_i(x_{-j})\\
    g_{n+1}(x) &= g'_n(x)+\frac{\varphi'_j(x_j) - c'_j(x)}{\varepsilon} g_n(x)
\end{align*}
where $g_1(x) = c'_j(x)$. $g(x)$ differs when $j=1,..,J$, but for clarity the subscript $j$ is omitted in $g(x)$.

Next we prove the following claim by induction on $n$:

\textit{$(P_n)$ For $i=0,...,k$, $k=0,...,n-2$, $\|g_{n-k}^{(i)}\|_\infty$ is bounded by a polynomial in $\frac{1}{\varepsilon}$ of order $n-k+i-1$.}

When $n=2$, ($i=0,k=0$),
\begin{align*}
    g_2(x)&=g'_1(x)+\frac{\varphi'_j(x_j) - c'_j(x)}{\varepsilon} g_1(x)\\
    \|g_2(x)\|_\infty &\leq \|g_1'(x)\|_\infty + \frac{\|\varphi'_j(x_j)\|_\infty + \|c'_j(x)\|_\infty}{\varepsilon} \|g_1(x)\|_\infty
\end{align*}
Let $C_j = \max_{i\geq 0}\|c_j^{(i)}(x)\|_\infty$. Since $\|\varphi_j\|_\infty<\infty$, let $C = \max\{C_1,...,C_J, K_\varepsilon\}$. Because $\mu_1,...,\mu_J$ are probability measures, $\|\varphi_j^{(n)}\|_\infty\leq C \|g_n(x)\|_\infty$. Hence $\|g_2(x)\|_\infty\leq a_0+a_1 \frac{1}{\varepsilon}$ for some constant coefficient $a_0, a_1$.

Assume that $(P_n)$ is true for some $n\geq 2$, i.e.~$\|g_{n-k}^{(i)}\|_\infty$ is bounded by some polynomial $Q_{n-k+i-1}(\frac{1}{\varepsilon}):=\sum_{i=0}^{n-k+i-1}a_i\left(\frac{1}{\varepsilon}\right)^i$. We want to show $(P_{n+1})$ is also true. 

Note that given the bound for the triangular array $\left\{\|g_{n-k}^{(i)}\|_\infty, i=0,...,k, k=0,..,n-2\right\}$ in $(P_n)$, we only need to show the additional terms $\left\{\|g_{n-k+1}^{(k)}\|_\infty, k=0,...,n-1\right\}$ having the claimed bound in $(P_{n+1})$.

When $k=n-1$,
\begin{align*}
    g_2^{(n-1)} &= g_1^{(n-1)} + \sum_{p=0}^{n-1}\left( \begin{array}{c}n-1 \\p 
    \end{array} \right) \frac{\varphi_j^{(p+1)} - c_j^{(p+1)}}{\varepsilon}g_1^{(n-p-1)} \\
    \|g_2^{(n-1)}\|_\infty &\leq C
    +\sum_{p=0}^{n-1}\left( \begin{array}{c}n-1 \\p 
    \end{array} \right)  \frac{C\|g_{p+1}\|_\infty + C}{\varepsilon} C
\end{align*}
$(P_n)$ ensures that $\|g_{p+1}\|_\infty \leq Q_{p}(\frac{1}{\varepsilon}),p=0,..,n-1$, hence $\|g_2^{(n-1)}\|_\infty\leq Q_{n}(\frac{1}{\varepsilon})$.

When $k<n-1$,
\begin{align*}
    \|g_{n+1-k}^{(k)}\|_\infty &\leq \|g_{n-k}^{(k+1)}\|_\infty + \sum_{p=0}^{k}\left( \begin{array}{c} k \\p 
    \end{array} \right) \frac{\|\varphi^{(p+1)}_j\|_\infty+\|c^{(p+1)}_j\|_\infty}{\varepsilon}
    \|g_{n-k}^{(k-p)}\|_\infty \\
    &\leq Q_{n}(\frac{1}{\varepsilon}) + \sum_{p=0}^{k}\left( \begin{array}{c} k \\p 
    \end{array} \right) \frac{Q_{p}(\frac{1}{\varepsilon})+ C}{\varepsilon} Q_{n-p-1}(\frac{1}{\varepsilon})\\
    &\leq Q_n(\frac{1}{\varepsilon})
\end{align*}
Hence the proof for $(P_n)$ is complete. $(P_n)$ implies that $\|\varphi_j^{(n)}\|_\infty\leq Q_{n-1}(\frac{1}{\varepsilon})$ for any $n\geq 2$ and $j=1,..,J$, hence the optimal $\varphi$ is smooth.
\end{proof}

==> yuliang/Proof_thm1.tex <==
\newpage
\begin{proof}[Proof of Theorem \ref{thm:matching}]
We use the empirical process notations $\mathbb{P}_n f=\int f(x) \dd\bigotimes_{j=1}^J\hat\mu_{N_j}(x)$, $\mathbb{P} f=\int f(x) \dd\bigotimes_{j=1}^J\mu_{_j}(x)$, and $\mathbb{G}_Nf = \sqrt{N}(\mathbb{P}_Nf-\mathbb{P}f)$.
\begin{align*}
    &\sqrt{N}\left( \int f(x) \dd\hat\gamma_N(x) - \int f(x) \dd\gamma(x)  \right)\\
    &=\sqrt{N}\{ \mathbb{P}_N \hat K_N f - \mathbb{P} Kf \} \\
    &= \sqrt{N}\{ \mathbb{P}_N \hat K_Nf -\mathbb{P}\hat K_Nf +\mathbb{P}\hat K_Nf -\mathbb{P}Kf \}\\
    &=\mathbb{G}_N \hat K_Nf + \mathbb{P}\{ \sqrt{N}(\hat K_Nf-Kf) \}
\end{align*}
Now from Lemma \ref{lem:density}, $\sqrt{N}(\hat K_Nf-Kf)\rightsquigarrow Z_k f$ where $Z_k=\exp\left( \frac{\sum_j\varphi_j-c}{\varepsilon} \right) \frac{Z_\varphi}{\varepsilon}$ is a mean-zero tight Gaussian process. 
We first show that $\mathbb{G}_N \hat K_Nf\rightsquigarrow \mathbb{G}_pKf$ where $\mathbb{G}_pKf$ is a $\mathbb{P}$-Brownian bridge process indexed by $Kf$. Next, we show that $\mathbb{G}_N \hat K_Nf + \mathbb{P}\{ \sqrt{N}(\hat K_Nf-Kf) \}$ is a sequence of tight random functions. Finally we show that $\sqrt{N}\left( \int f(x) \dd\hat\gamma_N(x) - \int f(x) \dd\gamma(x)  \right)$ converges to a mean-zero tight process.

To show the convergence of $\mathbb{G}_N \hat K_Nf\rightsquigarrow \mathbb{G}_pKf$, we first verify the conditions in Lemma 19.24 in \cite{van2000asymptotic}.
Similar to the proof of Theorem \ref{thm:potential}, we define the following class of functions
\begin{align*}
    \tilde{\mathcal{F}}_{Kf}\coloneqq\left\{\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right) f \right]: \thickspace \right. \left.\thickspace \varphi\in \prod_jC^\infty(\mathcal{X}_j), f\in \prod_jC^{\alpha}(\mathcal{X}_j)\right\}
\end{align*}
Using the same argument as in Theorem \ref{thm:potential}, we split this class into $$\tilde{\mathcal{K}}_{K}\coloneqq\left\{\left[\exp\left(\frac{\sum_{j=1}^J\varphi_j - c}{\varepsilon}\right) \right]:\thickspace \right. \left.\thickspace \varphi\in \prod_jC^\infty(\mathcal{X}_j)\right\}$$ and $\tilde{\mathcal{G}}_{f}\coloneqq\left\{f: f\in \prod_jC^{\alpha}(\mathcal{X}_j)\right\}$. By Corollary 2.7.2 in \cite{wellner2013weak} and the assumption $d>2\alpha$, both $\tilde{\mathcal{K}}_{\delta,K}$ and $\tilde{\mathcal{G}}_{f}$ have bounded bracketing entropy integrals. Due to the compactness of $\mathcal{X}_j$ and smoothness of functions in $\tilde{\mathcal{K}}_{\delta,K}$ and $\tilde{\mathcal{G}}_{f}$, both classes are uniformly bounded $\mathbb{P}$-Donsker classes. Hence by Example 2.10.8 in \cite{wellner2013weak}, $\tilde{\mathcal{F}}_{\delta,Kf}$ is also $\mathbb{P}$-Donsker.

For any $\hat K_Nf\in \tilde{\mathcal{F}}_{\delta,Kf}$, by Lemma \ref{lem:consistency},
\begin{align*}
    \int_{\prod_j\mathcal{X}_j}& \left(\hat K_N(x)f(x)-K(x)f(x) \right)^2 \dd \mathbb{P}(x) 
    \leq \int_{\prod_j\mathcal{X}_j} \frac{1}{\epsilon^2}\left\| \sum_{j=1}^J\hat \varphi_{N_j}-\sum_{j=1}^J\varphi^*_j  \right\|_{\infty}^2 [K(x)f(x)]^2 \dd \mathbb{P}(x) \\
    &= o_p(1)
\end{align*}
By Lemma 19.24 in \cite{van2000asymptotic}, $\mathbb{G}_N \hat K_Nf\rightsquigarrow \mathbb{G}_pKf$.

It is easy to show that the linear mapping $\mathbb{P}$ is Hadamard-differentiable at any $f\in \prod_j L^\infty(\mathcal{X}_j)$
\begin{align*}
    \frac{\int_\mathcal{X}f+t_nh_n\dd\mathbb{P}-\int_\mathcal{X}f\dd\mathbb{P}}{t_n} \to \int_\mathcal{X}h\dd\mathbb{P}
\end{align*}
Hence $\mathbb{P}(\sqrt{N}(\hat K_N-K))f\rightsquigarrow \mathbb{P}Z_k f$.

===================(third try -> not right)=======================

Next, we use the extended continuous mapping, theorem 1.11.1 in \cite{wellner2013weak}, to show the weak convergence of the joint measure $\hat\gamma_N$ in a similar fashion as in the proof of Lemma 19.24 in \cite{van2000asymptotic}.

Define a function $g_n(z,h):=z\left(y_0+\frac{1}{\sqrt{n}}h\right) + \sqrt{n}\left(T_0(y_0+\frac{1}{\sqrt{n}}h) - T_0(y_0)\right)$. Assume that $g_n$ is defined on the domain $\mathbb{D}_n:=L^\infty(y_0+\frac{1}{\sqrt{n}}\mathcal{F}_n) \times \mathcal{F}_n$, where $\mathcal{F}_n:=\left\{h: y_0+\frac{1}{\sqrt{n}}h\in \prod_jC^\infty(\mathcal{X}_j)  \right\}$. In our case, choose $T_0 = \mathbb{P}\in L^\infty(\mathcal{F}_n)$, $y_0=K(x)\in \prod_jC^\infty(\mathcal{X}_j)$. It is easy to show that the linear mapping $T_0$ is Hadamard-differentiable at any $f\in \prod_j C^\infty(\mathcal{X}_j)$
\begin{align*}
    \frac{\int_\mathcal{X}f+t_nh_n\dd\mathbb{P}-\int_\mathcal{X}f\dd\mathbb{P}}{t_n} \to \int_\mathcal{X}h\dd\mathbb{P}
\end{align*}
as $t_n\to 0$ and $h_n\to h$, for $h_n,h\in \prod_j C^\infty(\mathcal{X}_j)$. Hence when $z_n\to z_0$ (in $L^\infty(\prod_j C^\infty(\mathcal{X}_j))$), $h_n\to h_0$ (in $L_2(T_0)$), $g_n(z_n,h_n)\to z_0(y_0)+T_0(h_0)$. 

Now apply $g_n(z_n,h_n)$ on $(\mathbb{G}_n, \sqrt{n}(\hat K_n-K) )$. From the previous part of the proof, we know that $(\mathbb{G}_n, \hat K_n)\rightsquigarrow (\mathbb{G}_p, K(x))$, and because $(\mathbb{G}_n, \sqrt{n}(\hat K_n-K) )$ only takes values on $\mathbb{D}_n$, which means that $\mathbb{G}_n$ only acts on $\hat K_n$, hence $(\mathbb{G}_n, \sqrt{n}(\hat K_n-K) )\rightsquigarrow (\mathbb{G}p, Z_k)$, by the extended continuous mapping theorem, 
\begin{align*}
    g_n(\mathbb{G}_n, \sqrt{n}(\hat K_n-K) ) & \rightsquigarrow \mathbb{G}_p(K) + \mathbb{P}Z_k
\end{align*}



% ==========================================


% Define a function $g_n(x,y):=x(\frac{1}{\sqrt{n}}y+c_1) + \mathbb{C}_2(y)$ on the product space $L^\infty(\mathcal{F}_1)\times \mathcal{F}_{2,N}$. Here, we can choose $\mathcal{F}_1:=\left\{ Kf:K\in \prod_jC^\infty(\mathcal{X}_j), f\in \prod_jC^{\alpha}(\mathcal{X}_j) \right\}$, $\mathcal{F}_{2,N}:=\left\{\sqrt{N}(f-c_1): f\in \mathcal{F}_1 \right\}$, and choose $c_1:=K(x)f(x)\in\mathcal{F}_1$, $\mathbb{C}_2:=\mathbb{P}\in L^\infty(\mathcal{F})$. 
% % Denote $L_N(\mathcal{F}_1):=\left\{ \sqrt{N}(\mathbb{P}_N-\mathbb{P})f: f\in \mathcal{F}_1 \right\}$. Then $L_N(\mathcal{F}_1)\times \mathcal{F}_{2,N} \subset L^\infty(\mathcal{F}_1)\times \mathcal{F}_{2,N}$.
% By the same argument as the previous proof, $\mathcal{F}_1$ is a $\mathbb{P}$-Donsker class.

% Denote $\mathcal{Y}_N = \sqrt{N}(\hat K_Nf - Kf)$, and $\frac{1}{N}\mathcal{Y}_N+c_1$ belongs to the Donsker class $\mathcal{F}_1$, $\mathbb{G}_N\rightsquigarrow \mathbb{G}_p$ on $\mathcal{F}_1$, and $\mathcal{Y}_N\rightsquigarrow Z_kf$ by Lemma  \ref{lem:density}.

% ==========================================

%  We can choose $c_1:=K(x)f(x)\in\mathcal{F}$, and $\mathbb{C}_2:=\mathbb{P}\in L^\infty(\mathcal{F})$. Define $\mathcal{D}_N\subset \mathcal{F}$ as 
% \begin{align*}
%      \mathcal{D}_N\coloneqq &\left\{ \left( \mathbb{G}_N, \mathcal{Z}_N\right):\mathbb{G}_Nh = \sqrt{N}(\mathbb{P}_Nh-\mathbb{P}h) \text{ for all } h\in \mathcal{F},  \mathcal{Z}_N:= \sqrt{N}(K_Nf-Kf),\right. \\
%      &K_N(x):= \left[\exp\left(\frac{\sum_{j=1}^J\varphi_{N_j} - c}{\varepsilon}\right) f \right], \|\varphi_N - \varphi^*\|_{C^k}<\delta_N\thickspace \forall k\in\mathbb{N}^d_0 \left.\thickspace \varphi\in \prod_jC^\infty(\mathcal{X}_j), f\in \prod_jC^{\alpha}(\mathcal{X}_j)\right\}
% \end{align*}
% $\delta_N\to 0$ as $N\to \infty$.  When $x_n\to x_0$
\end{proof}

==> yuliang/old_corollary3B.tex <==
For part B, denote $y(j,X)=f_j(X) = \mathbb{E}\{Y(j)|X\}$
\begin{align*}
    \mathbb{E}Y(j) &= \int_{\mathcal{X}_j} f_j(x_j)\dd \mu_j(x_j)
    % + \int_{\mathcal{X}_j}\sum_{t\in [-j]}\int_{\mathcal{X}_t} f_t(x_t) \dd\gamma(x_t|x_j)\dd\mu_j(x_j)\\
    % &=\int_{\mathcal{X}_j} f_j(x_j)\dd \mu_j(x_j)+
    % \int_{\mathcal{X}_j}\int_{\mathcal{X}_{[-j]}} \sum_{t\in [-j]} f_t(x_t)K(x_1,..,x_J)\dd\mu_{[-j]}(x_{[-j]})\dd\mu_j(x_j)\\
    % &=\int_{\mathcal{X}}\left(\sum_{j=1}^J f_j(x_j) \right) K(x)\dd\bigotimes_{j=1}^J\mu_{j}(x_j)
\end{align*}
In addition, for any $t\neq j$, 
\begin{align*}
    \mathbb{E}_{X_t}\{ \mathbb{E}_{X_j}(y(j,X_j)|X_t)\} = 
    \mathbb{E}_{X_t}\{ y(j,X_t) \} = \mathbb{E}_{X_t}\{ \mathbb{E}(Y(j)|X_t)\} = \mathbb{E}(Y(j))
\end{align*}
Now we can write the sample version in Definition \ref{def:matching_po1} as
\begin{align}\label{eq:cor1}
    &\mathbb{\hat E} Y(j)I(D(j)=1) + \mathbb{\hat E} \sum_{t\neq j}\int_{\mathcal{X}_j} Y(j,x)\dd\hat\gamma_{\epsilon,j|t}(x|X) I(D(t)=1) 
    % \\
    % &= \mathbb{\hat E}_{Y}Y(j)I(D(j)=1) + \mathbb{\hat E}_{Y} \sum_{t\neq j}Y(j)I(D(t)=1) 
    % \\
    % &= \int_{\prod_{j=1}^J \mathcal{X_j}}y(j,X_j)\dd\hat\gamma_N(x_1,..,x_J) + \int_{\prod_{j=1}^J \mathcal{X_j}} \sum_{t\neq j} y(j,x_j)\dd\hat\gamma_N(x_1,..,x_J) \\
    % &= \int_{\prod_{j=1}^J \mathcal{X_j}} \sum_{t\neq j} y(j,x_j)\dd\hat\gamma_N(x_1,..,x_J) 
\end{align}
Note that $\mathbb{\hat E}$ assigns equal weight $\frac{1}{N}$ to each triplet $(Y_i,X_i,T_i)$. From part $A$, we know the weak convergence of $\int_{\mathcal{X}_j} y(j,x)\dd\hat\gamma_{\epsilon,j|t}(x|X)$ given $X$. Denote $ g_{j}^{(\epsilon)}(y,x,t):=\int_{\mathcal{X}_j} y(j,s)\dd\gamma_{\epsilon, j|t}(s|x)I(T=t)$. Now we can write a more general version of (\ref{eq:cor1}) as $\mathbb{\hat E} \hat g_j^{(\epsilon)}(Y,X,T)$.

By Assumption \ref{ass:asybal}, let $P_T$ be the discrete marginal distribution of treatment assignment $T$, where $P_T(T=j)=\rho_j$, and let $\hat P_T$ be the empirical marginal distribution where $\hat P_T(T=j)=\frac{N_j}{N}$, where $N=\sum_{j=1}^J N_j$. By assumption \ref{ass:causal}, $Y_i = \eta_i+y(T_i,X_i)$ where $\eta_i$ is the mean-zero i.i.d noise that is independent of $(T,X)$.

\begin{align*}
    & \sqrt{N}\left( \mathbb{\hat E}Y(j) - \mathbb{E}Y(j) \right) \\
    = & \sqrt{N}\left( \int_{[-j]} \int_{\mathcal{X}_t,t\neq j} \int_{\mathcal{X}_j} f_j(s)\dd\hat\gamma_{\varepsilon,j|t}(s|x_t)I(T=t)\dd\hat\mu_t\dd\hat P_T + \frac{N_j}{N}\int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j - \mathbb{E}(Y(j)) + \frac{1}{N}\sum_{i=1}^N \eta_i\right)\\
    = & \sqrt{N} \left( \left(1-\frac{N_j}{N}\right)\int_{\mathcal{X}} f_j(x_j)\dd\hat\gamma_{N}(x) +\frac{N_j}{N}\int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j(x_j)
    - P_T \int_{\mathcal{X}}f_j(x_j)\dd\gamma(x)\right) + \frac{1}{\sqrt{N}}\sum_{i=1}^N \eta_i
    % = & \sqrt{N} \left( \int_{[J]} \int_{\mathcal{X}_t,t\neq j} \int_{\mathcal{X}_j} f_j(s)\dd\hat\gamma_{\varepsilon,j|t}(s|x_t)I(T=t)\dd\hat\mu_t\dd\hat P_T + \int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j  \right.\\
    % &\left.\vphantom{\int_{[J]} \int_{\mathcal{X}_t,t\neq j} \int_{\mathcal{X}_j} f_j(s)\dd\hat\gamma_{\varepsilon,j|t}(s|x_t)I(T=t)\dd\hat\mu_t\dd\hat P_T + \int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j  } - 
    % \int_{[J]}\right) + \sqrt{N}\frac{1}{N}\sum_{i=1}^N \eta_i\\
\end{align*}
The noise term $\frac{1}{\sqrt{N}}\sum_{i=1}^N \eta_i\rightsquigarrow N(0,1)$ independently from the first term. 
\begin{align*}
    &\sqrt{N} \left( \left(1-\frac{N_j}{N}\right)\int_{\mathcal{X}} f_j(x_j)\dd\hat\gamma_{N}(x) +\frac{N_j}{N}\int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j(x_j)
    - P_T \int_{\mathcal{X}}f_j(x_j)\dd\gamma(x)\right)\\
    =& \sqrt{N} \left( \left(1-\frac{N_j}{N}\right)\int_{\mathcal{X}} f_j(x_j)\hat K_{N}(x)\dd\bigotimes_j\hat\mu_{N_j}(x) + \frac{N_j}{N}\int_{\mathcal{X}_j}f_j(x_j)\dd\hat\mu_j(x_j)
    - \int_{\mathcal{X}}f_j(x_j)\dd\gamma(x)\right)\\
    =& \sqrt{N} \left( \int_{\mathcal{X}} f_j(x_j) \left[ \left(1-\frac{N_j}{N}\right)\hat K_{N}(x) +\frac{N_j}{N} \right]\dd\bigotimes_j\hat\mu_{N_j}(x) 
    - \int_{\mathcal{X}}f_j(x_j)K(x)\dd\bigotimes_j\mu_{j}(x)\right)\\
    =& \sqrt{N} \left( \int_{\mathcal{X}} f_j(x_j) \left[ \left(1-\frac{N_j}{N}\right)\hat K_{N}(x) +\frac{N_j}{N} \right]\dd\bigotimes_j\hat\mu_{N_j}(x) 
    - \int_{\mathcal{X}}f_j(x_j)\left\{(1-\rho_j)K(x)+\rho_j\right\}\dd\bigotimes_j\mu_{j}(x)\right)\\
    &\rightsquigarrow G_jf_j
\end{align*}
The last step follows the same method as the proof of Corollary \ref{corr:matching}, by replacing $\hat K_N$ with $(1-N_j/N)\hat K_n+N_j/N$, and replacing $K$ by $(1-\rho_j)K + \rho_j$. 

The weak convergence of Definition \ref{def:matching_po1} now becomes 
\[\sqrt{N}\left\{ \mathbb{\hat E}\hat g_{N,j}^{(\epsilon)} - \mathbb{E}  g_{j}^{(\epsilon)}\right\} \rightsquigarrow G_j.\]

The rest of the proof follows the same method as the proof of Theorem 1.

==> yuliang/unused.tex <==
The matching estimator we propose can be extended to multiple treatment, hence we extend Assumption \ref{ass:causal} to the case where the treatment assignment represents a group of treatment on a group of individuals.\ndfg{I think we might call this not Assumption 5, because it does not replace Assumption 4, but is more general. Maybe we should call it 4'. Do you have a better idea?}\yxcm{Totally agree, will change this later.}
\begin{assumption}\label{ass:causal_general}
    For a group $G$ of individuals $\{l_1,..,l_{N_g}\}\subset \{1,...,N\}$, let random variable $D$ supported on $\{0,1\}^J$ be the binary representation of the treatment assignment for group $G$, let $D(j)$ be the $j$-th index in the vector $D$. $D(j)=1$ if treatment $j$ is assigned to group $G$.
\begin{enumerate}%[label = \roman*)]
    \item (Unconfoundedness) $D\perp Y |X$.
    \item (Overlap) $P(D(j)=1|X)$ is bounded away from 0 and 1.
    \item Let $\mathcal{T}=\{j: D(j)=1\}$ be the index set of the assigned treatment to group $G$. 
        \begin{enumerate}
            \item Given $D$ such that $\mathcal{T}=\{1,..,J\}$, assume that the probability measure induced by $X$ is $\gamma(x_1,..,x_J)$, supported on $\prod_{j=1}^J\mathcal{X}_j$;
            \item Given $D$ such that $\mathcal{T}^c = \{j: D(j)=0\}$ is not empty, and suppose there are $k$ elements in $\mathcal{T}$, sorted in ascending order, denoted by $\mathcal{T}(1),..,\mathcal{T}(k)$. Let $\pi_{\mathcal{T}}:\prod_{j=1}^J \mathcal{X}_j\to \prod_{j\in \mathcal{T}}\mathcal{X}_j$ be the project map, i.e. $\pi_{\mathcal{T}}(x_1,...,x_J) = (x_{\mathcal{T}(1)},...,x_{\mathcal{T}(k)})$. Then the measure induced by $X$ is assumed to be $\gamma_{\mathcal{T}}:=\gamma \circ \pi_{\mathcal{T}}^{-1}$.
        \end{enumerate}
     \item Given $D$, there exists a bounded continuous function $f_{\mathcal{T}}$ supported on $\prod_{j\in\mathcal{T}}\mathcal{X}_j$ such that $Y(\mathcal{T}) = f_{\mathcal{T}}(X)+\epsilon$. Here we denote $y(\mathcal{T},X):=f_{\mathcal{T}}(X)$ and $Y(\mathcal{T},X) = f_{\mathcal{T}}(X)+\epsilon$.
\end{enumerate}
\end{assumption}
The first two assumptions in Assumptions \ref{ass:causal} and \ref{ass:causal_general} are the same. Assumption \ref{ass:causal_general}.3 defines the joint distribution $\gamma$ of $X$ given all treatments are assigned to group $G$, and the marginal distributions $\gamma_{\mathcal{T}}$ when a subgroup of treatment is assigned to the group $G$. Combining Assumption \ref{ass:causal}.3 and Assumption \ref{ass:causal_general}.3, we can see that $\mu_j$ is the marginal distribution for $\gamma$ on $\mathcal{X}_j$.

\yxcm{$Y(j)$'s are correlated through $X_j$'s. We should be able to know the joint distribution of $Y(1),...,Y(J)$ given $\gamma$, but conditional on $D$.}

\yxcm{This sample version definition looks too complicated. We can remove it. But it can act as the comparison to \ref{eq:kmeans_po}}



The next definition is given for the potential outcome under a group of treatment.
\yxcm{Def 2 requires either (1) multiple treatment can be assigned to the same individual, which is more than the constraint for the optimal transport; or (2) $Y(\tau,X)$ is known as a function of $X$, which is usually unknown.}
\begin{definition}[Group treatment potential outcome]\label{def:matching_po2}
Suppose $D$ is supported on $\{0,1\}^J$. For a constant $J$ dimensional vector $\tau \in \{0,1\}^J$, let $\mathcal{I}_\tau$ be the index set $\{j:\tau(j)=1\}$, and $\mathcal{I}_\tau^c = [J]\setminus \mathcal{I}_\tau$.
Under the joint distribution $\gamma$ on $\prod_{j=1}^J\mathcal{X}_j$, denote $\gamma(x_\tau)$ as the (joint) marginal distribution on $\prod_{j\in \mathcal{I}_\tau}\mathcal{X}_j$, and $\gamma(x_{\tau_1}|x_{\tau_2})$ as the conditional distribution on $\prod_{j\in \mathcal{I}_{\tau_1}}\mathcal{X}_j$ given $X_{\tau_2}$.
Then under Assumption \ref{ass:causal_general},
\begin{align}
    Y(\mathcal{I}_\tau)&= \mathbb{E}_X\left( Y(\mathcal{I}_\tau,X)I(D=\tau) \right) +
     \mathbb{E}_X\left( Y(\mathcal{I}_\tau,X)I(D \neq \tau) \right)\\
     &= \int_{ \mathcal{X}_{\mathcal{I}_\tau} }  Y(\mathcal{I}_\tau,X) \dd\gamma(x_\tau) +
      \int_{ \mathcal{X}_{\mathcal{I}_\tau} } \int_{\mathcal{X}_{\mathcal{I}_\tau^c} } Y(\mathcal{I}_\tau^c,X) \dd\gamma(x_{\tau^c}|x_\tau) \dd\gamma(x_\tau) \label{eq:g_potential_2}
\end{align}
\end{definition}
The second equation \ref{eq:g_potential_2} is due to the fact that for any $D\neq \tau$, the corresponding $X$ either follows $\gamma(x_{\tau^c}|x_\tau)$, or follows a marginal in $\gamma(x_{\tau^c}|x_\tau)$. For example, when $J=5$, $\mathcal{I}_\tau = \{2,4,5\}$, then for some $D=(1,0,1,0,1)$, $\gamma(x_{(1,3,5)}|x_{(2,4,5)}) = \gamma(x_{(1,3)}|x_{(2,4,5)})$, and when $D = (0,0,1,0,1)$, $\gamma(x_{(3,5)}|x_{(2,4,5)})$ is a marginal of $\gamma(x_{(1,3)}|x_{(2,4,5)})$.

It is worth noting that in Definition \ref{def:matching_po2}, there is no assumption for the correlation structure of the treatment assignment random vector $D$. This means that our approach takes into account the correlation in $D$. 
